Avoiding local minima in multilayer network optimization by incremental training

Training a large multilayer neural network can present many difficulties due to the large number of useless stationary points. These points usually attract the minimization algorithm used during the training phase, which therefore results inefficient. Extending some results proposed in literature for shallow networks, we propose the mathematical characterization of a class of such stationary points that arise in deep neural networks training. Availing such a description, we are able to define an incremental training algorithm that avoids getting stuck in the region of attraction of these undesirable stationary points.

==> old_material.tex <==

\section*{Hierarchical structure and critical points of the FNN model}
To simplify the analysis, we considered a FNN with a single hidden layer ($L = 1)$ with $H$ neurons and one output unit ($m = 1$). Therefore, we defined the FNN response to a generic input $x$ as
\begin{align*}
f^{(H)}(x; \theta^{(H)}) = & \sum_{j=1}^{H}v_{j} g\biggl(w_{j}^{T}x+w_{j0}\biggr) + v_0 \\
= & \sum_{j=1}^{H}v_{j} g\biggl(\Tilde{w_{j}}^{T}\Tilde{x}\biggr) + v_0, \hspace{0.5cm} \tilde{x} = [1\> \>x^T]^T, \> \> \tilde{w_{j}} = [w_{j0} \> \> w_{j}^T]^T
\end{align*}
where $v_j$ is the output weight of the arc connecting hidden neuron $j$ to the output node, $v_{0}$ is the output threshold, and 
$$\theta^{(H)} = [v_0 \> \> v_1 \ldots v_H \> \> \tilde{w_1}^T \ldots \tilde{w_H}^T]^T \in \mathbb{R}^{H(n+2)+1} = \Theta_H.$$
For a generic monotone activation function $g$, the mapping $\theta^{(H)} \mapsto f(\cdot)^{(H)}$ is not one to one. Indeed, the same $f(\cdot)^{(H)}$ is obtained if we exchange two neurons $(v_j, \tilde{w_j}) \rightleftharpoons (v_k, \tilde{w_k})$, or we change the sign of input output weights $(v_j, \tilde{w_j}) \rightarrow (-v_j, -\tilde{w_j})$. Thus, we can define the subset $\mathcal{S}_H$ of $\mathcal{F}$ as follows:
$$\mathcal{S}_H = \left\{f^{(H)}(x; \theta^{(H)}): \mathcal{R}^L \rightarrow \mathcal{R} \> | \> \theta^{(H)} \in \Theta_H\right\}$$
It is clear that $\mathcal{S}_{H-1} \subset \mathcal{S}_{H}$, but the embedding is not canonical. 
Without loss of generality, let us define a function $f^{(H-1)}(x; \theta^{(H-1)}) \in \mathcal{S}_{H-1}-\mathcal{S}_{H-2}$ as follows:
$$f^{(H-1)}(x; \theta^{(H-1)}) = \sum_{j=2}^{H}\zeta_{j} g\biggl(\Tilde{u_{j}}^{T}\Tilde{x}\biggr) + \zeta_0$$
Basically, there are three different kind of mappings of $\phi: \theta^{(H-1)} \mapsto \theta^{(H)}$ such that 
$$f^{(H)}(x; \phi(\theta^{(H-1)})) = f^{(H-1)}(x; \theta^{(H-1)}).$$ The first one is obtained whenever we reset one of the output weights $v_j$ 
$$\alpha_{\tilde{w}}: \theta^{(H)} = \left[\zeta_0 \> \> 0 \> \> \zeta_2 \> \ldots \> \zeta_H \> \> \tilde{w}^T \> \> \tilde{u}^{T}_2 \> \ldots \> \tilde{u}^{T}_H\right]^T, \quad \forall \tilde{w} \in \mathbb{R}^{n+1}.$$
The second kind of mapping is obtained by resetting one of the input weights $w_j$
$$\beta_{v, \xi}: \theta^{(H)} = \left[(\zeta_0 - v g(\xi)) \> \> v \> \> \zeta_2 \> \ldots \> \zeta_H \> \> (\xi \> 0^T) \>  \> \tilde{u}^{T}_2 \> \ldots \> \tilde{u}^{T}_H\right]^T, \quad \forall (v, \xi) \in \mathbb{R}^{2}.$$ The last one is defined as
$$\gamma_{\lambda}: \theta^{(H)} = \left[\zeta_0 \> \> \lambda \zeta_2 \> \> (1 - \lambda)\zeta_2 \> \> \zeta_3 \> \ldots \> \zeta_H \> \> \tilde{u}^{T}_2 \> \> \tilde{u}^T_2 \> \> \tilde{u}^{T}_3 \> \ldots \> \tilde{u}^{T}_H\right]^T, \quad \forall \lambda \in \mathbb{R}.$$
Now, let $\theta^{(H-1)}_{*}$ be a critical point of $$R_{emp}(\theta^{(H-1)})=\frac{1}{P}\sum_{p=1}^{P} \mathcal{L} (y^{p}, f^{H-1}(x^{p}, \theta^{(H-1)})).$$
The following equations hold
\begin{align}
    \label{deriv:eq_1}
    \frac{\partial R_{emp}(\theta^{(H-1)}_*)}{\partial \zeta_0} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H-1}(x^{p}, \theta^{(H-1)}_*))} = 0\\
    \label{deriv:eq_2}
    \frac{\partial R_{emp}(\theta^{(H-1)}_*)}{\partial \zeta_j} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H-1}(x^{p}, \theta^{(H-1)}_*))} g(\tilde{u}^T_{j*} \tilde{x}^p) = 0, \quad j = 2, \ldots, H \\
    \label{deriv:eq_3}
    \frac{\partial R_{emp}(\theta^{(H-1)}_*)}{\partial u_j} & = \frac{1}{P} \sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H-1}(x^{p}, \theta^{(H-1)}_*))} {\zeta_{j*} g^\prime(\tilde{u}^T_{j*} \tilde{x}^p)} (\tilde{x}^p)^T = 0^T, \quad j = 2, \ldots, H
\end{align}
Let us now consider the analogous derivatives of $R_{emp}(\theta^{(H)})$ with respect to a generic $\theta^{(H)}$.
\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H)})}{\partial v_0} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta^{(H)}))} \\
    \frac{\partial R_{emp}(\theta^{(H)})}{\partial v_j} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta^{(H)}))} g(\tilde{w}^T_{j} \tilde{x}^p), \quad j = 1, \ldots, H \\
    \frac{\partial R_{emp}(\theta^{(H)})}{\partial w_j} & = \frac{1}{P} \sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta^{(H)}))} v_{j}{g^\prime(\tilde{w}^T_{j} \tilde{x}^p)} (\tilde{x}^p)^T, \quad j = 1, \ldots, H\\
\end{align*}
Note that $f^{(H)}(x^p; \theta^{(H)}) = f^{(H-1)}(x^p; \theta^{(H-1)}_*)$ by choosing either $\theta^{(H)} = \gamma_{\lambda}(\theta^{(H-1)}_*)$ or $\theta^{(H)} = \beta(0, \xi)(\theta^{(H-1)}_*)$ and taking into account that $\alpha_{\tilde{w}} = \beta(0, \xi)$ with $\tilde{w} = (\xi \> \> 0^T)^T$. 

First, let us note that, when $\theta^{(H)} = \beta(0, \xi)(\theta^{(H-1)}_*)$, recalling (\ref{deriv:eq_1}),
\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H)})}{\partial v_1} & = \frac{1}{P}g(\xi)\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta^{(H)}))}  = 0,\\
    \frac{\partial R_{emp}(\theta^{(H)})}{\partial w_1} & = \frac{1}{P} \sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta^{(H)}))} \cdot 0\cdot{g^\prime(\xi)} (\tilde{x}^p)^T = 0\\
\end{align*}
On the other hand, when $\theta^{(H)} = \gamma_{\lambda}(\theta^{(H-1)}_*)$, recalling (\ref{deriv:eq_2}) and (\ref{deriv:eq_3}), we have
\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H)})}{\partial v_1} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta^{(H)}))} g(\tilde u_{2*}^T \tilde x^p) = 0,\\ 
    \frac{\partial R_{emp}(\theta^{(H)})}{\partial w_1} & = \frac{1}{P} \sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta^{(H)}))} \lambda \zeta_{2*}{g^\prime(\tilde{u}^T_{2*} \tilde{x}^p)} (\tilde{x}^p)^T=0.\\
\end{align*}



Note that all of the other partial derivatives, for $j=2,\dots,H$, are zero, thus defining critical points of $R_{emp}(\theta^{(H)})$. These points lie on lines in $\theta^{(H)}$ as $\lambda$ and $w$ vary.

%\section{Augmenting the width of a single layer FNN}
\par\medskip

\subsection{Adding a set of $K$ neurons}
Now, we generalize the above results by  adding more than one neuron at the same time in the hidden layer. Therefore, let's recall the response of a FNN with $H+K$ neurons along with the empirical risk
\begin{align*}
f^{(H+K)}(x; \theta^{(H+K)}) = & \sum_{j=1}^{H+K}v_{j} g\biggl(\Tilde{w_{j}}^{T}\Tilde{x}\biggr) + v_0, \hspace{0.5cm} \tilde{x} = [1\> \>x^T]^T.
\end{align*}

$$R_{emp}(\theta^{(H+K)})=\frac{1}{P}\sum_{p=1}^{P} \mathcal{L} (y^{p}, f^{H+K}(x^{p}, \theta^{(H+K)})).$$

First of all, we extended the mapping $\alpha_{\tilde w}$ by setting to zero the weights of the outputs of the newly added neurons. 
\begin{align*}
\alpha_{\tilde{w}}: \theta^{(H+K)} & = \left[\zeta_0 \> \> \zeta_1 \> \> \zeta_2 \> \ldots \> \zeta_H \> \> \underbrace{0 \> \> \ldots \> \> 0}_{K\ \mbox{\scriptsize weights}} \tilde{u}^T_1 \> \> \tilde{u}^{T}_2 \> \ldots \> \tilde{u}^{T}_H   \> \tilde w^T_1 \> \ldots \> \tilde w^T_K\>\right]^T  \\
& \forall \tilde{w}_i \in \mathbb{R}^{n+1},\quad i=1,\dots, K.
\end{align*}
The second kind of mapping is obtained by resetting one of the input weights $w_j$
\begin{align*}
\beta_{v, \xi}: \theta^{(H+K)} & = \left[(\zeta_0 - \sum_{i=1}^Kv_i g(\xi_i)) \> \> \zeta_1 \> \ldots \> \zeta_H \> v_1 \> \ldots \> v_K \> \> \tilde{u}^{T}_1 \> \ldots \> \tilde{u}^{T}_H \> (\xi_1 \> 0^T) \> \ldots \> (\xi_K \> 0^T) \right]^T\\
 &  \forall v_i, \xi_i \in \mathbb{R}, \ i=1,\dots,K
\end{align*}
The last one is defined as
\begin{align*}\gamma_{\lambda}: \theta^{(H+K)} & = \left[\zeta_0, \> \> \zeta_1, \> \> \ldots \> \lambda_{0}\zeta_H, \> \lambda_1 \zeta_H ,\> \ldots \> \lambda_K \zeta_H,\> \> \> \tilde{u}^T_1, \> \> \ldots \> \tilde{u}^{T}_H, \> \underbrace{\tilde u_H^T, \> \ldots \> \tilde u_H^T}_{K\ \mbox{\scriptsize vectors}}\right]^T\\
&  \forall \lambda_i \in \mathbb{R},\ i=0,\dots,K,\ \sum_{i=0}^{K}\lambda_i = 1.
\end{align*}
With the above transformations, it holds that
\begin{equation}\label{responsehpk}
  f^{(H+K)}(x;\phi(\theta^{(H)})) = f^{(H)}(x;\theta^{(H)})
\end{equation}
when $\phi(\cdot)$ is either $\alpha_{\tilde w}$ or $\beta_{v,\xi}$ or $\gamma_\lambda$.
\par\smallskip


Considering the neural network with $H$ units and the expressions of the derivatives of $R_{emp}(\theta^{(H)})$ when $\theta_*^{(H)}$ is stationary, we have
\begin{align}
\label{deriv1:eq1}
    \frac{\partial R_{emp}(\theta_*^{(H)})}{\partial v_0} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta_*^{(H)}))} = 0\\
\label{deriv1:eq2}
    \frac{\partial R_{emp}(\theta_*^{(H)})}{\partial v_j} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta_*^{(H)}))} g(\tilde{w}^T_{*,j} \tilde{x}^p)=0, \quad j = 1, \ldots, H \\
\label{deriv1:eq3}
    \frac{\partial R_{emp}(\theta_*^{(H)})}{\partial w_j} & = \frac{1}{P} \sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta_*^{(H)}))} v_{*,j}{g^\prime(\tilde{w}^T_{*,j} \tilde{x}^p)} (\tilde{x}^p)^T=0, \quad j = 1, \ldots, H
\end{align}
Now for the augmented network, i.e. with parameters $\theta^{(H+K)}$, we have
\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_0} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H+K}(x^{p}, \theta^{(H+K)}))} \\
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_j} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H+K}(x^{p}, \theta^{(H+K)}))} g(\tilde{w}^T_{j} \tilde{x}^p), \quad j = 1, \ldots, H+K \\
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial w_j} & = \frac{1}{P} \sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H+K}(x^{p}, \theta^{(H+K)}))} v_{j}{g^\prime(\tilde{w}^T_{j} \tilde{x}^p)} (\tilde{x}^p)^T, \quad j = 1, \ldots, H+K\\
\end{align*}
Then, we can state the following proposition.
\begin{proposition}
Every stationary point  $\theta_*^{(H)}$ of $R_{emp}(\theta^{(H)})$ corresponds to stationary points for $R_{emp}(\theta^{(H+K)})$ when $\theta^{(H+K)} = \beta_{(0,\xi)}(\theta_*^{(H)})$ or $\theta^{(H+K)} = \gamma_{\lambda}(\theta_*^{(H)})$.
\label{prop3.1}
\end{proposition}

{\bf Proof}.
Recalling (\ref{responsehpk}) and (\ref{deriv1:eq1}), we have
\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_0} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta_*^{(H)}))} = 0,\\
%
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_j} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta_*^{(H)}))} g(\tilde{w}^T_{*,j} \tilde{x}^p)= 0, \quad j = 1, \ldots, H \\
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial w_j} & = \frac{1}{P} \sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta_*^{(H)}))} v_{*,j}{g^\prime(\tilde{w}^T_{*,j} \tilde{x}^p)} (\tilde{x}^p)^T = 0, \quad j = 1, \ldots, H\\
\end{align*}
Considering again (\ref{responsehpk}) and (\ref{deriv1:eq1}), we have for $j=H+1,\dots,H+K$ and when $\theta^{(H+K)} = \beta_{(0,\xi)}(\theta_*^{(H)})$ that
\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_j} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta_*^{(H)}))} g(\xi_{j-H}) = 0, \\
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial w_j} & = \frac{1}{P} \sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta_*^{(H)}))} \cdot 0 \cdot{g^\prime(\xi_{j-H})} (\tilde{x}^p)^T=0.
\end{align*}

Instead, recalling (\ref{responsehpk}), (\ref{deriv1:eq2}) and (\ref{deriv1:eq3}),  we have when $\theta^{(H+K)} = \gamma_{\lambda}(\theta^{(H)})$ that

\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_j} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta_*^{(H)}))} g(\tilde{w}^T_{*,H} \tilde{x}^p)=0, \\
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial w_j} & = \frac{1}{P} \sum_{p=1}^{P} { \mathcal{L}^\prime(y^{p}, f^{H}(x^{p}, \theta_*^{(H)}))} \lambda_{j-H}v_{*,H}{g^\prime(\tilde{w}^T_{*,H} \tilde{x}^p)} (\tilde{x}^p)^T=0.
\end{align*}

$\hfill\Box$



\par\medskip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Networks with $m>1$ outputs}

Now, we generalize the above results by adding more than one neuron at the same time in the hidden layer when we have more than one output unit. Therefore,  let's recall the response of a FNN with $H+K$ neurons along with the empirical risk
\begin{align*}
f_r^{(H+K)}(x; \theta^{(H+K)}) = & \sum_{j=1}^{H+K}v_{jr} g\biggl(\Tilde{w_{j}}^{T}\Tilde{x}\biggr) + v_{0r}, \hspace{0.5cm} \tilde{x} = [1\> \>x^T]^T.
\end{align*}

$$R_{emp}(\theta^{(H+K)})=\frac{1}{P}\sum_{p=1}^{P} \mathcal{L} (y^{p}, f^{H+K}(x^{p}, \theta^{(H+K)})),$$
where $v_{jr}$ is the output weight of the arc connecting hidden neuron $j$ to the output node $r$, $v_{0r}$ the bias of the output node $r$, $y^p\in\Re^m$, $i=1,\dots,P$ and $f^{H+K}:\Re^n\to\Re^m$.
\par\smallskip

First of all, we extended the mapping $\alpha_{\tilde w}$ by setting to zero the weights of the outputs of the newly added neurons.

\begin{align*}
\alpha_{\tilde{w}}: \theta^{(H+K)} & = \left[\zeta_0 \> \> \zeta_1 \> \> \zeta_2 \> \ldots \> \zeta_H \> \> \underbrace{0 \> \> \ldots \> \> 0}_{K\ \mbox{\scriptsize $m$-zero vectors}} \tilde{u}^T_1 \> \> \tilde{u}^{T}_2 \> \ldots \> \tilde{u}^{T}_H   \> \tilde w^T_1 \> \ldots \> \tilde w^T_K\>\right]^T  \\
& \forall \tilde{w}_i \in \mathbb{R}^{n+1},\quad i=1,\dots, K,
\end{align*}
where $\zeta_j\in\Re^m$, $j=0,\dots,H$.

The second kind of mapping is obtained by resetting one of the input weights $w_j$
\begin{align*}
\beta_{v, \xi}: \theta^{(H+K)} & = \left[(\zeta_0 - \sum_{i=1}^Kv_i g(\xi_i)) \> \> \zeta_1 \> \ldots \> \zeta_H \> v_1 \> \ldots \> v_K \> \> \tilde{u}^{T}_1 \> \ldots \> \tilde{u}^{T}_H \> (\xi_1 \> 0^T) \> \ldots \> (\xi_K \> 0^T) \right]^T\\
 &  \forall v_i, \xi_i \in \mathbb{R}, \ i=1,\dots,K
\end{align*}
where $v_j\in\Re^m$, $j=0,\dots,K$.

The last one is defined as
\begin{align*}\gamma_{\lambda}: \theta^{(H+K)} & = \left[\zeta_0, \> \> \zeta_1, \> \> \ldots \> \lambda_{0}\zeta_H, \> \lambda_1 \zeta_H ,\> \ldots \> \lambda_K \zeta_H,\> \> \> \tilde{u}^T_1, \> \> \ldots \> \tilde{u}^{T}_H, \> \underbrace{\tilde u_H^T, \> \ldots \> \tilde u_H^T}_{K\ \mbox{\scriptsize vectors}}\right]^T\\
&  \forall \lambda_i \in \mathbb{R},\ i=0,\dots,K,\ \sum_{i=0}^{K}\lambda_i = 1.
\end{align*}
With the above transformations, it holds that
\begin{equation}\label{responsehpk}
  f_r^{(H+K)}(x;\phi(\theta^{(H)})) = f_r^{(H)}(x;\theta^{(H)}),\qquad r=1,\dots,m 
\end{equation}
when $\phi(\cdot)$ is either $\alpha_{\tilde w}$ or $\beta_{v,\xi}$ or $\gamma_\lambda$.
\par\smallskip


Considering the neural network with $H$ units and the expressions of the derivatives of $R_{emp}(\theta^{(H)})$ when $\theta_*^{(H)}$ is stationary, we have
\begin{align}
\label{deriv1:eq1}
    \frac{\partial R_{emp}(\theta_*^{(H)})}{\partial v_{0r}} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y_r^{p}, f_r^{H}(x^{p}, \theta_*^{(H)}))} = 0,\qquad r=1,\dots,m\\
\label{deriv1:eq2}
    \frac{\partial R_{emp}(\theta_*^{(H)})}{\partial v_{jr}} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y_r^{p}, f_r^{H}(x^{p}, \theta_*^{(H)}))} g(\tilde{w}^T_{*,j} \tilde{x}^p)=0, \quad j = 1, \ldots, H,\ r=1,\dots,m, \\
\label{deriv1:eq3}
    \frac{\partial R_{emp}(\theta_*^{(H)})}{\partial w_j} & = \frac{1}{P} \sum_{p=1}^{P}\sum_{r=1}^{m} { \mathcal{L}^\prime(y_r^{p}, f_r^{H}(x^{p}, \theta_*^{(H)}))} v_{*,jr}{g^\prime(\tilde{w}^T_{*,j} \tilde{x}^p)} (\tilde{x}^p)^T=0, \quad j = 1, \ldots, H
\end{align}

Now for the augmented network, i.e. with parameters $\theta^{(H+K)}$, we have
\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_{0r}} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y_r^{p}, f_r^{H+K}(x^{p}, \theta^{(H+K)}))},\qquad r=1,\dots,m \\
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_{jr}} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y_r^{p}, f_r^{H+K}(x^{p}, \theta^{(H+K)}))} g(\tilde{w}^T_{j} \tilde{x}^p), \quad j = 1, \ldots, H+K,\ r=1,\dots,m, \\
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial w_j} & = \frac{1}{P} \sum_{p=1}^{P}\sum_{r=1}^{m} { \mathcal{L}^\prime(y_r^{p}, f_r^{H+K}(x^{p}, \theta^{(H+K)}))} v_{jr}{g^\prime(\tilde{w}^T_{j} \tilde{x}^p)} (\tilde{x}^p)^T, \quad j = 1, \ldots, H+K\\
\end{align*}

Then, we can state the following proposition.

\begin{proposition}
Every stationary point  $\theta_*^{(H)}$ of $R_{emp}(\theta^{(H)})$ corresponds to stationary points for $R_{emp}(\theta^{(H+K)})$ when $\theta^{(H+K)} = \beta_{(0,\xi)}(\theta_*^{(H)})$ or $\theta^{(H+K)} = \gamma_{\lambda}(\theta_*^{(H)})$.
\label{prop4.1}
\end{proposition}

{\bf Proof}.
Recalling (\ref{responsehpk}) and (\ref{deriv1:eq1}), we have
\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_{0r}} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y_r^{p}, f_r^{H}(x^{p}, \theta_*^{(H)}))} = 0,\qquad r=1,\dots,m,\\
%
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_{jr}} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y_r^{p}, f_r^{H}(x^{p}, \theta_*^{(H)}))} g(\tilde{w}^T_{*,j} \tilde{x}^p)= 0, \quad j = 1, \ldots, H,\ r=1,\dots,m, \\
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial w_j} & = \frac{1}{P} \sum_{p=1}^{P}\sum_{r=1}^{m} { \mathcal{L}^\prime(y_r^{p}, f_r^{H}(x^{p}, \theta_*^{(H)}))} v_{*,jr}{g^\prime(\tilde{w}^T_{*,j} \tilde{x}^p)} (\tilde{x}^p)^T = 0, \quad j = 1, \ldots, H\\
\end{align*}
Considering again (\ref{responsehpk}) and (\ref{deriv1:eq1}), we have for $j=H+1,\dots,H+K$ and when $\theta^{(H+K)} = \beta_{(0,\xi)}(\theta_*^{(H)})$ that 

\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_{jr}} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y_r^{p}, f_r^{H}(x^{p}, \theta_*^{(H)}))} g(\xi_{j-H}) = 0,\qquad r=1,\dots,m, \\
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial w_j} & = \frac{1}{P} \sum_{p=1}^{P}\sum_{r=1}^{m} { \mathcal{L}^\prime(y_r^{p}, f_r^{H}(x^{p}, \theta_*^{(H)}))} \cdot 0 \cdot{g^\prime(\xi_{j-H})} (\tilde{x}^p)^T=0.
\end{align*}

Instead, recalling (\ref{responsehpk}), (\ref{deriv1:eq2}) and (\ref{deriv1:eq3}),  we have when $\theta^{(H+K)} = \gamma_{\lambda}(\theta^{(H)})$ that

\begin{align*}
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial v_{jr}} & = \frac{1}{P}\sum_{p=1}^{P} { \mathcal{L}^\prime(y_r^{p}, f_r^{H}(x^{p}, \theta_*^{(H)}))} g(\tilde{w}^T_{*,H} \tilde{x}^p)=0, \qquad r=1,\dots,m,\\
    \frac{\partial R_{emp}(\theta^{(H+K)})}{\partial w_{jr}} & = \frac{1}{P} \sum_{p=1}^{P}\sum_{r=1}^{m} { \mathcal{L}^\prime(y_r^{p}, f_r^{H}(x^{p}, \theta_*^{(H)}))} \lambda_{j-H}v_{*,H}{g^\prime(\tilde{w}^T_{*,H} \tilde{x}^p)} (\tilde{x}^p)^T=0.
\end{align*}
$\hfill\Box$

The critical points in Propositions \ref{prop3.1} and \ref{prop4.1} do not cover all of the critical points of $R_{emp}$. We consider the special subset of the critical points which appears because of the hierarchical structure of the model.

